Modular GPU Programming with Typed Perspectives

To achieve peak performance on modern GPUs, one must balance two frames of mind: issuing instructions to individual threads to control their behavior, while simultaneously tracking the convergence of many threads acting in concert to perform collective operations like Tensor Core instructions. The tension between these two mindsets makes modular programming error prone. Functions that encapsulate collective operations, despite being called per-thread, must be executed cooperatively by groups of threads. In this work, we introduce Prism, a new GPU language that restores modularity while still giving programmers the low-level control over collective operations necessary for high performance. Our core idea is typed perspectives, which materialize, at the type level, the granularity at which the programmer is controlling the behavior of threads. We describe the design of Prism, implement a compiler for it, and lay its theoretical foundations in a core calculus called Bundl. We implement state-of-the-art GPU kernels in Prism and find that it offers programmers the safety guarantees needed to confidently write modular code without sacrificing performance.

==> 1-introduction.tex <==
\section{Introduction}



\mb{This is not true, though fun to say. I need to think of a middle ground way of saying this.}

% On CPUs, (generally-speaking) a poor understanding of the hardware is a matter
% of performance, not correctness. Programmer is shielded from various concerns.
% \begin{itemize}
%     \item Caches manage access to memory
%     \item Visibility to different cores is somewhat transparently managed 
% \end{itemize}

On CPUs, many low-level hardware details are hidden from the programmer.
Multi-level caches transparently manage fast memory access, branch
prediction and out-of-order execution reduce the burden of instruction
scheduling, and virtualization creates the illusion of unbounded compute
resources. A programmer's poor understanding of the physical hardware may result
in slow, not incorrect code.


% Unlike the CPU, on the GPU, programmers are exposed to the underlying hardware,
% and programming it requires a fundamental understanding of the hardware.
% \begin{itemize}
%     \item Software managed cache + visibility is burden the of the programmer
%     \item Explicitly map compute and data to parallel resources
%     \item Compute and memory actually go together (sort of need to figure out
%     how your compute structure implies usage of memory and vice-a-versa). 
%     \item Certain operations only make sense collectively
% \end{itemize}

GPUs, by contrast, expose low-level architectural details directly to the
programmer. Programmers must explicitly map their computations onto a finite set
of compute and memory resources, deciding how to distribute work across threads,
warps, and blocks, while carefully managing data to fit within registers,
shared memory, and global memory. Coarse-grained primitives like Tensor Cores,
combined with asynchrony, have made this mapping even more complex. As such, a
mistake in the user's mental model of the machine will not only be a matter of
performance, but of correctness.


To get both safety and efficiency, several languages have been proposed that
\textit{raise the level of abstraction}. Own the enitre machine through kenrel launches,
\text{organize the library using namespaces}. 

- raised the level of abstraction
- global kernel launches


High-level languages do exist that get good performance: but still not the same
performance as hand-written kernel.
\begin{itemize}
    \item Underlying machine model changes, and dropping to a lower level of
    abstraction makes sense (warpgroups with Hopper and Triton)
\item A lot of these performance tricks require ingenuity and we are also
    figuring how to use the machine best.
\end{itemize}

As such, people continue to write code in low-level lanaguages

Composition/Modularity is broken because you need to read documentation to
figure out what to do.
\begin{itemize}
    \item Use CUB as a starting point?
    \item Types are categorized using namespaces, the implicit invariants of that
    namespace are not enforced by the compiler.
    \item Designing this is actually quite hard. The CUB BlockReduce
    documentation\footnote{See \url{https://nvidia.github.io/cccl/cub/api/classcub\_1\_1BlockReduce.html\#id3}}
    mentions that reusing that piece of data requires manual synchronizations
\end{itemize}

Low-level languages are the solution: high-level languages continue to struggle
to get the best performance. While high-level languages may offer productivity,
and can enforce some guarantees by limiting it to a particular level of the
hierarchy (like Triton), the need to have a low-level kernel language that
performance engineers can program with remains.
\begin{itemize}
    \item DeepSeek? 
    \item Coarser-grained instructions 
    \item Introduction of asynchrony
    \item Critical to actually utilize most of the FLOPs that are on the machine.
\end{itemize}

Types of Problems:
\begin{itemize}
    \item Insufficient computational resources
    \item Incorrect Synchronization 
\end{itemize}

% There's a tension between control and efficiency: we want both. We have a
% low-level language that prevents bugs that arise from using the hardware
% incorrectly. Same abstraction as CUDA. Compute and memory go together. 

Rather than sacrificing low-level control for safety, we aim to make
fine-grained GPU programming both safe and compositional by design. Our core
insight is that GPU programmers naturally map computations onto different parts
of the hardware hierarchy, and unlike CUDA, that obscures this mapping, we can
expose it explicitly using the syntax of the language. Using this
information, we can check, at compile time, whether assumptions about compute
and memory resources contradict the context in which code is being executed. 

We introduce \name{}, a new GPU programming language that makes ownership of the
hardware hierarchy explicit through lexical scopes. Inspired by capability-based
systems and Rust’s affine type system for memory safety, \name{} extends these
concepts to GPU execution by modeling ownership of not only memory but also of
compute resources. In \name{}, ownership of compute resources is represented
syntactically and checked by a substructural type system. Functions declare the
resources they require, and  \name{} statically ensures that these resources can
be provided.

In this work, we argue that the fundamental problem at the heart of CUDA is that, while programmers explicitly map their computations onto the hardware hierarchy, this mapping is not recoverable from the CUDA program itself.


Our contributions:
\begin{enumerate}
    \item \textit{A new imperative programming language} that represents the
    GPU’s compute and memory hierarchy through lexical scopes.  \jwc{This needs to be punchier---``lexical scopes'' sounds relatively pedstrian.
    We should say something like ``tracks the GPU's compute and memory resources through type-level capabilities''.}
    \item \textit{Mechanisms for shaping compute and memory},
    including ways to shape threads into collective units and to lower memory
    into different regions of the hierarchy.  
    \jwc{I think this contribution should be folded into the bullet point above.
    Indeed, the ``mechanisms for shaping compute and memory'' are part of the
    programming language. Moreover, they're sorta part and parcel with the type-level capability tracking: something like ``the language includes constructs for partitioning compute and memory resources''}
    \item \textit{Structured asynchrony}, in which synchronization is
    enforced implicitly through patterns of resource usage, rather than through
    explicit barriers.  
    \jwc{Like the previous. ``CCuda also includes support for blackwell features like asynchony''}
    \item \textit{A soundness theorem}, proving that well-typed programs in
    \name{} never get stuck due to unmet or conflicting resource requirements.  
    \jwc{IMO this contrib should be about the formalism. ``We build a formal model of CCuda... we use it to prove a soundess theorem that says...''}
    \item \jwc{Evaluation section. ``we demonstrate that CCuda can express state of the art kernels, etc''}
\end{enumerate}

\jwc{Let's talk about how these contribs are structured, I think they need to be refactored somewhat.}



==> 3-simple-mma.tex <==
\begin{ccudaCode}
@prism("device")
@requires(thread[32])
def simple_mma(a: ptr(const(float)) @ thread[32], 
               b: ptr(const(float)) @ thread[32],
               c: ptr(float) @ thread[32]):

  with group(thread[32]):
    stride : int @ thread[32] = 8

    tid : int @ thread[1] = id()

    regA: uint32_t[4] @ thread[1]
    row_a : int @ thread[1] = tid / 4
    col_a : int @ thread[1] = tid % 4
    offsetA : int @ thread[1] = row_a * stride + col_a

    regA[0] = __float_as_uint(a[offsetA + 0])
    regA[1] = __float_as_uint(a[offsetA + 8 * stride]); 
    regA[2] = __float_as_uint(a[offsetA + 4]); 
    regA[3] = __float_as_uint(a[offsetA + 8 * stride + 4]); 

    regB: uint32_t[2] @ thread[1]
    row_b : int @ thread[1] = tid % 4
    col_b : int @ thread[1] = tid / 4
    offsetB : int @ thread[1] = row_b * stride + col_b

    regB[0] = __float_as_uint(b[offsetB + 0])
    regB[1] = __float_as_uint(b[offsetB + 4 * stride])

    regC: uint32_t[4] @ thread[1]
    regC[0] = 0
    regC[1] = 0
    regC[2] = 0
    regC[3] = 0

    # Now do MMA!
    intrinsic.mma(
      regA[0], regA[1], regA[2], regA[3],  
      regB[0], regB[1],
      regC[0], regC[1], regC[2], regC[3],
      out=[regC[0], regC[1], regC[2], regC[3]]
    )

    row_c : uint32_t @ thread[1] = tid / 4
    col_c : int @ thread[1] = tid % 4
    offsetC : int @ thread[1] = row_c * stride + 2 * col_c

    with partition(c, offset=offsetC, dimension=thread[1]) as c_thread:
      with group(thread[1]):
        c_thread[0] += __uint_as_float(regC[0])
        c_thread[1] += __uint_as_float(regC[1])
        c_thread[8 * stride] += __uint_as_float(regC[2])
        c_thread[8 * stride + 1] += __uint_as_float(regC[3])

  return
\end{ccudaCode}

==> 9-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

==> eval/6.4.tex <==
\subsection{RQ4: Can \name{} catch bugs that CUDA would otherwise allow?}

To 

==> figs/perspective-filter.tex <==
\begin{figure}
\centering
\begin{minipage}[t]{0.23\textwidth}
\centering
\begin{ccudaBox}
var1 : int @ thread[8]
var2 : int @ grid[1]
var4 : int @ thread[8]
var5 : int @ thread[32]
\end{ccudaBox}
\caption*{Column 1 caption}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.23\textwidth}
\centering
\begin{ccudaBox}

var2 : int @ grid[1]


\end{ccudaBox}
\caption*{Column 2 caption}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.23\textwidth}
\centering
\begin{ccudaBox}

var2 : int @ grid[1]

var5 : int @ thread[32]
\end{ccudaBox}
\caption*{Column 3 caption}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.23\textwidth}
\centering
\begin{ccudaBox}
var1 : int @ thread[8]
var2 : int @ grid[1]
var4 : int @ thread[8]
var5 : int @ thread[32]
\end{ccudaBox}
\caption*{Column 4 caption}
\end{minipage}
    
\caption{A four-column layout using \texttt{minipage} inside a figure.}
\label{fig:fourcol}
\end{figure}
